An LMP O(log n)-Approximation Algorithm for Node Weighted Prize Collecting Steiner Tree

In the node-weighted prize-collecting Steiner tree problem (NW-PCST) we are given an undirected graph $G=(V,E)$, non-negative costs $c(v)$ and penalties $\pi(v)$ for each $v \in V$. The goal is to find a tree $T$ that minimizes the total cost of the vertices spanned by $T$ plus the total penalty of vertices not in $T$. This problem is well-known to be set-cover hard to approximate. Moss and Rabani (STOC'01) presented a primal-dual Lagrangean-multiplier-preserving $O(\ln |V|)$-approximation algorithm for this problem. We show a serious problem with the algorithm, and present a new, fundamentally different primal-dual method achieving the same performance guarantee. Our algorithm introduces several novel features to the primal-dual method that may be of independent interest.

==> quota.tex <==
\section{Quota Problem}
In the \textit{quota problem}, given the node cost $c(v)$ and profit
$\pi(v)$ for each vertex $v$ and a quota value $Q$,
we are asked to find the minimum
cost subtree of the graph with total profit at least $Q$.
Using the \textit{Lagrangian Relaxation} method and our LMP algorithm
 for \nwpcst, we give an $O(\lg n)$ approximation algorithm for the quota problem. Moreover, we consider the rooted version of the problem, where 
we want to find such minimum subtree containing a root vertex $r$. 

First let us formulate the quota problem with the following linear program. 
% Similar to the \nwpcst formulation, the variable $x_v$ denotes whether  the node $v$ exists in the solution ($x_v = 1$) or not ($x_v = 0$) and  the variable $z_S$ for a subset $S \subseteq V'$ denotes whether $S$ is a set of excluded nodes from the solution when $z_S = 1$ and $z_S = 0$ otherwise.

\begin{align}
  \min \quad{} & \sum_{v \in V'} c(v)x_v
 \tag{Quota} \label{quota} \\
  \textrm{s.t.} \quad{} & \sum_{v\in \Gamma(S)} x_v + \sum_{U | S \subseteq U} z_U  \geq 1 && \forall S\subseteq V', \nonumber \\
  & x_v + \sum_{U | v\in U} z_U  \geq 1 && \forall v\in V', \nonumber \\
\label{const:quota}   & \sum_{S \subseteq V'} \pi(S) z_S \leq \sum_{v \in V'} \pi(v) - Q &&  \\
  & x_v \in \{0,1\} && \forall v \in V', \nonumber \\
  & z_S \in \{0,1\} && \forall S \subseteq V',
  \nonumber
\end{align}

\noindent The differences between the formulation above and the linear program \ref{primal} for prize collecting version are the quota constraint \ref{const:quota} and that in prize collecting problem we have penalty values in our objective function whereas here we do not.

Assume that we ignore the quota constraint and we allow all the solutions to deviate from the requested profit value $Q$, but in return we incur a penalty equal to $\lambda$ times the \textit{profit deviation} of the solution from the desired value $Q$ for an arbitrary real value $\lambda$.
Let $\Pi = \sum_{v \in V'}\pi(v)$. The profit deviation of a primal solution $(x,z)$ is defined as $\sum_{S \subseteq V'} \pi(S)z_S - (\Pi - Q)$, which is the difference between profit of the solution in comparison to $Q$ (a negative value if the solution has profit more than $Q$). This modification to our linear program gives us the Lagrangian Relaxation of the quota problem:

\begin{align}
  \min \quad{} & \sum_{v \in V'} c(v)x_v + \lambda(\sum_{S  \subseteq V'}\pi(S)z_S - (\Pi - Q)) 
 \tag{LRQuota} \label{lrquota} \\
  \textrm{s.t.} \quad{} & \sum_{v\in \Gamma(S)} x_v + \sum_{U | S \subseteq U} z_U  \geq 1 && \forall S\subseteq V', \nonumber \\
  & x_v + \sum_{U | v\in U} z_U  \geq 1 && \forall v\in V', \nonumber \\
  & x_v \in \{0,1\} && \forall v \in V', \nonumber \\
  & z_S \in \{0,1\} && \forall S \subseteq V',
  \nonumber
\end{align}

\noindent Writing the dual of the \ref{lrquota}, we get the following linear program denoted by \ref{lrquota-d}:

\begin{align} 
 \max \quad{} & \sum_{S \in V'} y_S + \sum_{v \in V'} p_v - \lambda(\Pi - Q) \tag{LRQuota-D}\label{lrquota-d} \\
\textrm{s.t.} \quad{}  &
\sum_{S | v\in \Gamma(S)} y_S + p_v \leq c(v)  &&  \forall v \in V' \notag \\
&  \sum_{U \subseteq S} y_S + \sum_{v \in S} p_v \leq \sum_{v \in S} \lambda\pi(v)  &&
 \forall S \subseteq V'\notag \\
& y \geq \0 \notag \\
& p \geq \0 \notag
\end{align}

\noindent Note that for any arbitrary $\lambda$,
every solution $(x,z)$ to the quota problem is a feasible solution 
for the relaxed version, so the optimal solution for the \ref{lrquota} 
problem is a lower bound for the quota problem. Therefore,
by weak duality, the value of any solution to the dual problem \ref{lrquota-d} is also not larger than the optimal solution of the quota problem. 

The dual formulation \ref{lrquota-d} differs from the dual of the  price collecting problem only in the constant value $-\lambda(\Pi - Q)$ added to objective function, so if we give an instance of the quota problem with 
penalty values $\pi'(v) = \lambda\pi(v)$ for each $v \in V'$, by 
the LMP property of the prize collecting algorithm (theorem \ref{thm:lmp}), 
it gives us a feasible solution $T$ with a dual solution $(y,p)$ to \ref{lrquota-d} such that:
$$
\sum_{v \in T} c_v + \alpha(n) \pi'(V'\setminus T) \leq \alpha(n)(\sum_{S \subseteq V'} y_S + \sum_{v\in V'} p_v) 
$$
Where $\alpha(n)$ is a function of order $\lg n$. For ease of notation let us denote the value $\sum_{S \subseteq V'} y_S + \sum_{v\in V'} p_v$  of the dual solution $(y,p)$ by $Y$ and denote $V'\setminus T$ by $\bar T$. So we have:
\begin{align}
\sum_{v \in T} c_v + \alpha(n) \lambda \pi(\bar T) \leq \alpha(n)Y. 
\label{eq:lmpness}
\end{align}
Subtracting $\alpha(n)\lambda(\Pi - Q)$ from both sides, we get:
\begin{align}
\sum_{v \in V'} c_v + \alpha(n) \lambda (\pi(\bar T) - \Pi + Q) & \leq \alpha(n)(Y - \lambda(\Pi-Q)) \nonumber \\
& \leq \alpha(n)OPT_Q \label{eq:optbound}
\end{align}

\noindent
Where the last inequality follows from the fact that the right hand side is 
the objective function of the dual LP \ref{lrquota-d} multiplied by $\alpha(n)$. For every $\lambda$, the prize collecting algorithm finds a feasible solution
 for the relaxed quota problem. If we can find a suitable $\lambda$ for which 
this solution has profit exactly equal to $Q$, then we have a feasible solution 
for the original quota problem and we are done. However the solution may
have profit less than or greater than $Q$. If we run the prize collecting algorithm for the $\lambda$ values equal to $0$ and a value large enough
we find two solutions with profit $0$ and $\Pi$ respectively. We may assume that $0 \leq Q \leq \Pi$, so there are always two values of $\lambda$, say
$\lambda_1$ and $\lambda_2$ and by binary searching we can make these two values close enough such that:
\begin{itemize}
\item The prize collecting algorithm gives us two solutions $T_1$ and 
$T_2$ and their corresponding dual solutions $(y^{(1)},p^{(1)})$ and 
$(y^{(2)},p^{(2)})$ for the relaxed quota problem with $\lambda$ value equal to $\lambda_1$ and $\lambda_2$ respectively, such that 
$\pi(T_1) \leq Q$ and $\pi(T_2) \geq Q$.

\item $\lambda_2 - \lambda_1 \leq \frac{OPT_Q}{\Pi}$. 
\end{itemize}

\noindent Note that we do not need to know the exact value of the $OPT_Q$,
instead we can continue the
binary search until $\lambda_2 - \lambda_1$ is less than a value which is certainly less than $OPT_Q$ such as the minimum non-zero cost
of all vertices.
We enumerate over all possible values of $OPT_Q$ and continue as follows. First remove every
vertex with node-cost distance more than $OPT_Q$ from $r$.
Clearly no such vertex exists in the optimal solution. Obtain two 
solutions $T_1$ and $T_2$ for the relaxed quota prblem with the above 
properties and \textit{merge} them as we will explain later.
Before getting to the merging procedure, we prove that a good convex
combination of the cost of the two solutions $T_1$ and $T_2$ 
is no greater than $O(\lg n)OPT_Q$.

Let $a_1$ and $a_2$ be two values such that $a_1 + a_2 = 1$
and they are proportional to the profit deviation of the solution 
$T_2$ to the solution $T_1$. More precisely, let
$$
a_1 = \frac{\pi(T_2) - Q}{\pi(T_2) - \pi(T_1)}, \,\,\,\,
a_2 = \frac{Q - \pi(T_1)}{\pi(T_2) - \pi(T_1)}.
$$

\begin{lem}
$a_1c(T_1) + a_2c(T_2) \leq O(\lg n) OPT_Q$.
\end{lem}
\begin{proof}
Since $a_1 + a_2 = 1$, the convex combination $(a_1y^{(1)} + a_2y^{(2)},a_1p^{(1)} + a_2p^{(2)})$ is a feasible solution for
\ref{lrquota-d} with $\lambda$ equal to $\lambda_2$ (note $\lambda_2 \geq \lambda_1$) and therefore $a_1Y^{(1)} + a_2Y^{(2)} - \lambda_2(\Pi - Q) \leq OPT_Q$.
By equation \ref{eq:lmpness} we have:
$$
a_1c(T_1) + a_2c(T_2) 
$$ $$
\leq \alpha(n)\big(a_1Y^{(1)} + a_2Y^{(2)} - (a_1\lambda_1\pi(\bar T_1) + a_2\lambda_2\pi(\bar T_2))\big)
$$ $$
\leq \alpha(n)\big(a_1Y^{(1)} + a_2Y^{(2)} - \lambda_2(a_1\pi(\bar T_1) + a_2\pi(\bar T_2)) + (\lambda_2 - \lambda_1)\pi(\bar T_2)\big)
$$

\noindent By the definition of $a_1$ and $a_2$, we have $a_1\pi(\bar T_1) + a_2\pi(\bar T_2) = a_1(\Pi - \pi(T_1)) + a_2(\Pi - \pi(T_2)) = \Pi - Q$,  so,
\begin{align}
a_1c(T_1) + a_2c(T_2) &\leq \alpha(n)\big(OPT_Q+ (\lambda_2 - \lambda_1)\pi(\bar T_2)\big) \nonumber \\
& \leq \alpha(n)\big(OPT_Q + \frac{OPT_Q}{\Pi} \Pi) \nonumber \\
& = 2\alpha(n)OPT_Q \nonumber
\end{align}
\end{proof}

It only remains to show that given the the trees $T_1$ and $T_2$, how to
merge them to find a tree with profit at least $Q$ and cost 
$O(\lg n)OPT_Q$.
%We consider two cases, if $a_2 \geq \frac{1}{2}$,  then by the lemma above, $c(T_2) \leq 2\alpha_2c(T_2) = O(\lg n)OPT_Q$ and the tree $T_2$ has already profit at least $Q$, so $T_2$ satisfies our condition and we are done. 

%If $a_2 \leq \frac{1}{2}$,
Our final solution consists of the vertices of $T_1$ supplemented by some vertices of $T_2$ with profit at least $q = Q - \pi(T_1)$.
First, identify all of the vertices of $T_1$ to a vertex $r'$ to obtain a graph
$G'$. Let $T_2'$ be the corresponding vertices of $T_2$ in $G'$. Note that both $T_1$ and $T_2$ are connected subgraphs in $G$, 
so the vertices of $T_2'$, which are $V(T_1) \setminus V(T_2) \cup \{r'\}$, form a connected subgraph of $G'$ and also we have $\pi(T_2') \geq  \pi(T_2) - \pi(T_1) \geq q$.
We call a subgraph $S$ \textit{cost-effective}, if
$\frac{c(S)}{\pi(S)} \leq \frac{c(T_2')}{\pi(T_2')}$. 
Starting with the cost-effective tree $T' = V(T_2')$ in $G'$, 
continue the following procedure (which keeps $T'$ a cost-effective connected subgraph) while it changes the graph $T'$: \\
Select an edge $e$ from $T'$ with non-leaf vertices at both ends,
let $S$ and $R$ be the two components of $T'$ after removing the edge $e$. At least one of $S$ or $R$ are cost-effective. For each cost-effective subgraph $S$ or $R$, say $S$, do the following:
\begin{enumerate}
\item If $\pi(S) \geq q$, remove $R$ from $T'$.
\item If $\pi(S) < q$, identify all vertices of $S$ to a super node $S$ and
set the cost and the profit of the super vertex $S$ equal to the total cost and 
total profits of the vertices of $S$, respectively.
\end{enumerate}
It is easy to see that at the end, $T'$ is a cost-effective star graph with
profit at least $q$.
\begin{lem}
There is a connected subgraph $T''$ of $T'$ with profit at least $q$ and cost at most $O(\lg n)OPT_Q$.
\end{lem}
\begin{proof}
If a set $S$ is cost-effective, and has size no more than $O(1)q$, then by the previous lemma and the definition of a cost-effective set we have:
$$ c(S) \leq \pi(S)\frac{c(T_2')}{\pi(T_2')} \leq O(1)q\frac{c(T_2')}{\pi(T_2')} \leq O(1)(Q-\pi(T_1))\frac{c(T_2')}{\pi(T_2')}  $$
$$ \leq O(1)(Q-\pi(T_1))\frac{c(T_2')}{\pi(T_2) - \pi(T_1)}
\leq O(1)a_2c(T_2') $$
$$ \leq O(1)a_2c(T_2)   = O(\lg n)OPT_Q.$$

During the procedure above, we never identify a subgraph to a super vertex
if the subgraph has profit more than $q$ or if it is not cost-effective. Therefore, every super vertex $S$ is cost-effective and has cost 
$ O(\lg n)OPT_Q$. Moreover, at the beginning, we removed every vertex with cost more than $OPT_Q$. So regardless of a vertex being an original vertex or a super vertex, it does not have cost more than $O(\lg n)OPT_Q$. 

If there is a vertex $v$ in $T'$ with profit at least $q$, the single vertex $v$ is the desired subgraph. Also, if the total profit of $T'$ is not more than 
$2q$, then since $T'$ is cost effective $T'$ has cost $O(\lg n)OPT_Q$
and we are done. 
Now suppose that every vertex has profit less than $q$
and $T'$ has profit more than $2q$, then $T'$ has at leas $3$ vertices. Suppose that $T'$ consists of a 
vertex $u$ of degree more than $1$ and all other vertices in $T'$
are leaves adjacent to $u$. For an arbitrary vertex $v \in V(T') \setminus \{u\}$, by removing the edge $uv$ from $T'$, we have a 
single vertex $v$ and a star $R$ with profit more than $q$. Since none
of the cases 1 and 2 were applicable, $R$ is not cost-effective, hence $\{v\}$ is cost-effective. By our arbitrary choice of $v$, we conclude that every vertex in $T'$ except $u$ is cost-effective.

Consider an empty set $U$
and add adjacent vertices of $u$ in $T'$ to $U$ until $U \cup \{u\}$ induces a subgraph of $T'$ with profit at least $q$. Note that $U$ does not have profit more than $2q$ and it is cost effective. So by the arguments above $c(U \cup \{u\}) = O(\lg n)OPT_Q$ and it is connected and we are done. 
\end{proof}

Finally, if the supplemental subgraph $T''$ provided by the procedure above and previous lemma is not connected to the root, add a minimum cost path
$P$ from root to $T''$.  The graph $T_1 \cup T''$ has profit at least 
$q + \pi(T_1) = Q$ and cost $O(\lg n)OPT_Q$ and satisfies our quota problem constraints.
Note that $P$ has cost at most $OPT_Q$ since we have removed every 
vertex from the graph with node-cost distance more than $OPT_Q$ at the 
beginning. 
